Reducing Property Graph Queries to Relational Algebra for Incremental View Maintenance

The property graph data model of modern graph database systems is increasingly adapted for storing and processing heterogeneous datasets like networks. Many challenging applications with near real-time requirements -- e.g. financial fraud detection, recommendation systems, and on-the-fly validation -- can be captured with graph queries, which are evaluated repeatedly. To ensure quick response time for a changing data set, these applications would benefit from applying incremental view maintenance (IVM) techniques, which can perform continuous evaluation of queries and calculate the changes in the result set upon updates. However, currently, no graph databases provide support for incremental views. While IVM problems have been studied extensively over relational databases, views on property graph queries require operators outside the scope of standard relational algebra. Hence, tackling this problem requires the integration of numerous existing IVM techniques and possibly further extensions. In this paper, we present an approach to perform IVM on property graphs, using a nested relational algebraic representation for property graphs and graph operations. Then we define a chain of transformations to reduce most property graph queries to flat relational algebra and use techniques from discrimination networks (used in rule-based expert systems) to evaluate them. We demonstrate the approach using our prototype tool, ingraph, which uses openCypher, an open graph query language specified as part of an industry initiative. However, several aspects of our approach can be generalised to other graph query languages such as G-CORE and PGQL.

==> alg-grouping-criteria.tex <==
\SetKwFunction{KwFnDGC}{DetermineGroupingCriteria}
\begin{algorithm}[htb]
  \DontPrintSemicolon
  \KwData{E is the list of elements in the \lstreturn\ or \lstwith\ clause}
  \Fn{\KwFnDGC{E}}{
    $G \leftarrow \{\}$ \tcp*[r]{initial set of grouping criteria}
    $Q \leftarrow Q \union E$ \tcp*[r]{queue of expressions to process}
    \While{Q is not empty} {
      $q \leftarrow \mathrm{pop}(Q)$\;
      \uIf(\tcp*[f]{vertex, edge or property}){q is a variable}{
        $G \leftarrow G \union \{q\}$ \;
      }
      \uElseIf{q is a non-grouping function}{
        $Q \leftarrow Q \union \mathrm{arguments}\left(q\right)$ \tcp*[r]{add each argument}
      }
      \ElseIf(\tcp*[f]{list, map, etc.}){q is a composite expression}{
        $Q \leftarrow Q \union \{q\}$ \tcp*[r]{add each element}
      }
    }
    \Return $G$
  }
  \caption{Determine grouping criteria from return item list.}
  \label{alg:grouping-criteria}
\end{algorithm}


==> compilation.tex <==
\section{Compilation}

\newcommand*\numcircledmod[1]{\tikz[baseline=(char.base)]{\node[shape=rounded rectangle,rounded corners=1pt,draw,inner sep=1.2pt] (char) {#1};}}
\newcounter{mapping}[section]
\newcommand{\mapping}[1]{\refstepcounter{mapping}\numcircledmod{\themapping}\label{ctr:#1}}
\newcommand{\refmapping}[1]{\numcircledmod{\autoref{ctr:#1}}}

In this section, we present relational graph algebra using the examples of \autoref{sec:language-constructs} and provide a mapping that allows compilation from \opencypher constructs to this algebra.

\subsection{An Algebra for Formalising Graph Queries}
\label{sec:rga}

We present both standard operators of relational algebra~\cite{DBLP:books/daglib/0006733} and operators for graph relations. We follow the \opencypher query language and present a mapping from the language constructs to their algebraic equivalents, summarized in \autoref{table:operators}. The corresponding rows of the table (\eg \refmapping{getvertices}) are referred from the text.


\subsubsection{Basic operators.}

The \emph{\projectiontext} operator $\projectionop$ keeps a specific set of attributes in the relation: $ t = \projection{\atom{x_1}, \ldots, \atom{x_n}}{} \left(r\right).$ Note that the tuples are not deduplicated (\ie filtered to sets), thus $t$ will have the same number of tuples as $r$. The projection operator can also rename the attributes, \eg $\projection{\atom{x1} \assign \atom{y1}}{} \left(r\right)$ renames $\atom{x1}$ to $\atom{y1}$.

The \emph{\selectiontext} operator $\selectionop$ filters the incoming relation according to some criteria. Formally,
$ t = \selection{\theta} \left(r\right), $
where predicate $\theta$ is a propositional formula. Relation $t$ contains all tuples from $r$ for which $\theta$ holds.

\subsubsection{Vertices and patterns.} \refmapping{getvertices}--\refmapping{getverticeslabels} The \emph{\getverticestext}~\cite{DBLP:conf/edbt/HolschG16} nullary operator $\getvertices{v}{l_1 \land \ldots \land l_n}$ returns a graph relation of a single attribute $v$ that contains vertices that have \emph{all} of labels $l_1, \ldots, l_n$. Using this operator, the query in \autoref{lst:get-vertices} is compiled to
\input{adbis/relalg-get-vertices}

\refmapping{patterni}--\refmapping{patterniv} The \emph{\expandouttext} unary operator $\expandout{v}{w}{l_1 \land \ldots \land l_n}{e}{t_1 \lor \ldots \lor t_k}{1}{1}(r)$ adds new attributes $e$ and $w$ to each tuple iff there is an edge $e$ from $v$ to $w$, where
$e$ has \emph{any} of types $t_1, \ldots, t_k$, while
$w$ has \emph{all} labels $l_1, \ldots, l_n$.
More formally, this operator appends the $\tuple{e, w}$ to a tuple iff $\verticestoedges(e) = \tuple{v, w}$, $\atom{l_1}, \ldots, \atom{l_n} \in l_w$ and $t_e \in \{\atom{t_1}, \ldots, \atom{t_k}\}$. Using this operator, the query in \autoref{lst:expand-out} can be formalised as
\input{adbis/relalg-expand-out}

Similarly to the \expandouttext operator, the \emph{\expandintext} operator~$\expandinop$ appends $\tuple{e, w}$ iff $\verticestoedges(e) = \tuple{w, v}$, while the \emph{\expandbothtext} operator~$\expandbothop$ uses edge $e$ iff either $\verticestoedges(e) = \tuple{v, w}$ or $\verticestoedges(e) = \tuple{w, v}$.
We also propose an extended version of this operator, $\expandout{v}{w}{}{e}{}{min}{max}$, which may use between $\atom{min}$ and $\atom{max}$ hops.
Using this extension, \autoref{lst:multihop} is compiled to
\input{adbis/relalg-multihop}



\subsubsection{Combining and filtering pattern matches.}

\refmapping{matchi}--\refmapping{optionalmatchii} In order to express the uniqueness criterion for edges (illustrated in \autoref{sec:oc-uniqueness}) in a compact way, we propose the \emph{\alldifferenttext} operator. The \alldifferenttext operator $\alldifferent{E_1, \ldots, E_n}{(r)}$ filters $r$ to keep tuples where variables in $\cup_{i} E_{i}$ are pairwise different.
It can be expressed as a \selectiontext:
$$\alldifferent{E_1, \ldots, E_n}{(r)} = \selection{ \hspace{-3.2ex} \bigwedge\limits_{\substack{e_1, e_2 \in \cup_{i} {E_i} \\ e_1 \neq e_2}} { \hspace{-3.8ex} r.e_1 \,\neq\, r.e_2 } }{(r)}$$

\noindent Using the \alldifferenttext operator, query in \autoref{lst:alldifferent} is compiled to
\input{adbis/relalg-alldifferent}

\refmapping{matchi}--\refmapping{matchii}
The result of the \emph{\jointext} operator $\joinop$ is determined by creating the \cartesianproducttext of the relations, then filtering those tuples which are equal on the attributes that share a common name. The combined tuples are projected: from the attributes present in both of the two input relations, we only keep the ones in $r$ and drop the ones in $s$. Thus, the join operator is defined as
$$r \join s = \pi_{R \union S} \left(\selection{r.A_1 = s.A_1\,\land\,\ldots\,\land\,r.A_n = s.A_n)} \left(r \times s\right) \right),$$
where $ \{ A_1, \ldots, A_n \} = R \intersection S $ is the set of attributes that occur both in $R$ and $S$.

\noindent In order to allow pattern matches share the same edge, they must be included in different \lstinline+MATCH+ clauses as shown on \autoref{lst:non-unique-edges} which is compiled to
\input{adbis/relalg-non-unique-edges}





The query in \autoref{lst:join} with two patterns in one \lstinline|MATCH| clause is compiled to:
\input{adbis/relalg-join}


\refmapping{optionalmatchi}--\refmapping{optionalmatchii} The \emph{\leftouterjointext} operator produces $t = r \leftouterjoinop s$ combining matching tuples of $r$ and $s$ according to a given matching semantics.\footnote{Matching semantics might use value equality of attributes that share a common name (similarly to \jointext) to use an arbitrary condition (similarly to $\theta$-join).} In case there is no matching tuple in $s$ for a particular tuple $e \in r$, $e$ is still included in the result, with tuple attributes that exclusively belong to relation $s$ having a value of $\relnull$.



\subsubsection{Result and subresult operations.}

\refmapping{returnii} The \emph{\duplicateeliminationtext} operator $\duplicateeliminationop$ eliminates duplicate tuples in a bag.

\refmapping{returniii} The \emph{\groupingtext} operator $\groupingop$ groups tuples according to their value in one or more attributes and aggregates the remaining attributes.

We generalize the \groupingtext operator to explicitly state the \emph{grouping criteria} and allow for complex aggregate expressions.
This is similar to the SQL query language where the grouping criteria is explicitly given in \texttt{GROUP BY}.

We use the notation $\grouping{e_1, e_2, \ldots }{c_1, c_2, \ldots }$, where $c_1, c_2, \ldots $ in the superscript form the \emph{grouping criteria}, \ie the list of expressions whose values partition the incoming tuples into groups. For each and every group this aggregation operator emits a single tuple of expressions listed in the subscript, \ie $\tuple{e_1, e_2, \ldots }$.
Given attributes $a_j \in \{a_1, \ldots, a_n\}$ of the input relation, $c_i$ is an arithmetic expression of $a_j$ attributes, while $e_i$ is an expression built from $a_j$ attributes using the common arithmetic operators and grouping functions.

\input{alg-grouping-criteria}

We have discussed aggregation semantics on \opencypher in \autoref{sec:aggregation}. Formal algorithm for determining the grouping criteria is given in \autoref{alg:grouping-criteria}.
Building on this algorithm and the \groupingtext operator, \autoref{lst:grouping} is compiled to

\input{adbis/relalg-grouping}


\subsubsection{Unwinding and list operations.}


\refmapping{unwind} The \emph{\unwindtext}~\cite{botoeva_et_al:LIPIcs:2018:8607} operator $\unwind{xs \assign x}$ takes the list in attribute $\atom{xs}$ and unfolds it to an attribute $\atom{x}$, as demonstrated in \autoref{fig:unwind}. Using this operator, the query in \autoref{lst:unwind} can be formalised as
\input{adbis/relalg-unwind}

\refmapping{orderby} The \emph{\sorttext} operator $\sortop$ transforms a bag relation of tuples to a list of tuples by ordering them. The ordering is defined for selected attributes and with a certain direction for each of them (ascending $\asc$/descending $\desc$), \eg $\sortop_{\asc \atom{x1}, \desc \atom{x2}} (r)$.

\refmapping{top} The \emph{\toptext} operator $\topp{l}{s}$ (adapted from~\cite{DBLP:conf/sigmod/LiCIS05}) takes a list as its input, skips the first $s$ tuples and returns the next $l$ tuples.\footnote{SQL implementations offer the \texttt{OFFSET} and the \texttt{LIMIT}/\texttt{TOP} keywords.}

Using the \sorttext and \toptext operators, the query of \autoref{lst:duplicate-elimination-sorting} is compiled to:
\input{adbis/relalg-duplicate-elimination-sorting}

\subsubsection{Combining results.}

The $\unionop$ operator produces the \emph{set union} of two relations, while the $\bagunionop$ operator produces the \emph{\baguniontext} of two operators, \eg $\{\tuple{1, 2}, \tuple{3, 4}\} \bagunionop \{\tuple{1, 2}\} = \{\tuple{1, 2}, \tuple{1, 2}, \tuple{3, 4}\}$. For both the \uniontext and \baguniontext operators, the schema of the operands must have the same attributes.




\setlength\extrarowheight{2.5pt}
\setlength\tabcolsep{3.6pt}
\begin{table*}[htbp]
	\begin{adjustbox}{center}
	\input{table-compilation}
	\end{adjustbox}
	\caption{Mapping from \opencypher constructs to relational algebra. Variables, labels, types and literals are typeset as \lstinline|<<v>>|. The notation \lstinline|<p>p</p>| represents patterns resulting in a relation $p$, while \lstinline|[[r]]| stands for a relation $r$ that is a results of the previous query parts. To avoid confusion with the ``\lstinline+..+'' language construct (used for ranges), we use ``\lstinline+...+'' to denote omitted query parts.}
	\label{table:mapping}
\end{table*}

\subsection{Mapping openCypher Queries to Graph Relational Algebra}
\label{sec:compilation}

In this section, we first give the mapping algorithm of \opencypher queries to \rga, then we give a more detailed listing of the compilation rules for the query language constructs in \autoref{table:mapping}. We follow a bottom-up approach to build the \rga expression.

\begin{enumerate}
\item
Process each query part as follows and combine their result using the \uniontext opertaion. As the \uniontext operator is technically a binary operator, the \uniontext of more than two query parts are represented as a left deep tree of \lstinline+UNION+ operators.

\item For each subquery of a query part, denoted by $\atom{t}$ the \rga tree built from the prefix of subqueries up to but not including the current subquery, process the current subquery as follows.

\setlength\tabcolsep{3.6pt}
\begin{enumerate}
	\item A single pattern is turned left-to-right to a \getverticestext for the first vertex and a chain of \expandintext, \expandouttext or \expandbothtext operators for inbound, outbound or undirected relationships, respectively.
	\item Comma-separated patterns in a single \lstinline+MATCH+ are connected by \jointext.
	\item Append an \alldifferenttext operator for all edge variables that appear in the \lstinline+MATCH+ clause because of the non-repeating edges language rule.
	\item Process the \lstinline+WHERE+ subclause of a single \lstinline+MATCH+ clause.
	\item Several \lstinline+MATCH+ clauses are connected to a left deep tree of \jointext.

	      For \lstinline+OPTIONAL MATCH+, \leftouterjointext is used instead of \jointext. In case there is a \lstinline+WHERE+ subclause, condition given there is part of the join condition, \ie it will never filter on the input from previous \lstinline+MATCH+ clauses.
	\item If there is a positive or negative pattern deferred from \lstinline+WHERE+ processing, append it as a \jointext or a combination of \leftouterjointext and \selectiontext operator filtering on no matches were found, respectively.
	\item If this is not the first subquery, combine the curent subquery with the \rga tree of the preceding subqueries by appending a \jointext here. Its left operand will be $\atom{t}$ and its right operand will be the \rga tree built so far from the current subquery.
	\item Append \groupingtext, if \lstinline+RETURN+ or \lstinline+WITH+ clause has grouping functions inside.
	\item Append \projectiontext operator based on the \lstinline+RETURN+ or \lstinline+WITH+ clause. This operator will also handle the renaming (i.e. \lstinline+AS+).
	\item Append \duplicateeliminationtext operator, if the \lstinline+RETURN+ or \lstinline+WITH+ clause has the \lstinline+DISTINCT+ modifier.
	\item Append a \selectiontext operator if \lstinline+WITH+ had the optional \lstinline+WHERE+ subclause.
\end{enumerate}
\end{enumerate}

\subsection{Summary and Limitations}

In this section, we presented a mapping that allows us to express the example queries of \autoref{sec:language-constructs} in graph relational algebra. We extended relational algebra by adapting operators ($\getverticesop$, $\expandoutop$, $\sortop$, $\topop$), precisely specifying grouping semantics ($\groupingop$) and defining the all-different operator ($\alldifferentop$). Finally, we proposed an algorithm for compiling \opencypher graph queries to graph relational algebra.

Our mapping does not completely cover the \opencypher language. As discussed in \autoref{sec:opencypher}, some constructs are defined as legacy and thus were omitted. The current formalisation does not include expressions (\eg conditions in selections) and maps. Compiling data manipulation operations (such as \mbox{\lstinline+CREATE+}, \mbox{\lstinline+DELETE+}, \mbox{\lstinline+SET+,} and \mbox{\lstinline+MERGE+}) to relational algebra is also subject of future work.


==> opencypher.tex <==
\section{The openCypher Query Language}
\label{sec:opencypher}

Cypher is the a high-level declarative graph query language of the Neo4j graph database. It allows users to specify graph patterns by a syntax resembling an actual graph, which makes the queries easy to comprehend.

The goal of the \opencypher project~\cite{openCypher} is to provide a standardised specification of the Cypher language.
In the following, we introduce features of the language using examples.

\subsection{Language Constructs}
\label{sec:language-constructs}

\subsubsection{Inputs and outputs.} \opencypher queries take a \emph{property graph} as their input, however the result of a query is not a graph, but a \emph{graph relation}.

\subsubsection{Vertex and path patterns.}

The basic building blocks of queries are patterns of vertices and edges.
\autoref{lst:get-vertices} shows a query that returns all vertices that model a \textsf{Person}. The query in \autoref{lst:expand-out} matches two \textsf{Persons} connected by a \textsf{KNOWS} edge and returns the names of each pair. Query given on \autoref{lst:multihop} describes person pairs that know each other directly or has a friend in common, \ie from person $\atom{p1}$, the other person $\atom{p2}$ can be reached using one or two hops.

\listingcypher{get-vertices}{Getting vertices}

\listingcypher{expand-out}{Pattern matching}

\listingcypher{multihop}{Variable length path}

\listingcypher{grouping}{Grouping}

\subsubsection{Filtering.}

Pattern matches can be filtered in two ways as illustrated in \autoref{lst:selection1} and \autoref{lst:selection2}. (1) Vertex and edge patterns in the \lstinline+MATCH+ clause might have vertex label/edge type constraints, and (2) the optional \lstinline+WHERE+ subclause of \lstinline+MATCH+ might hold predicates.

\listingcypher{selection1}{Filtering for edge property}

\listingcypher{selection2}{Filtering}

\subsubsection{Unique and non-unique edges.}
\label{sec:oc-uniqueness}

A \lstinline+MATCH+ clause defines a graph pattern. A query can be composed of multiple patterns spanning multiple \lstinline+MATCH+ clauses. For matches of a pattern within a single \lstinline+MATCH+ clause, edges are required to be unique.
However, matches for multiple \lstinline+MATCH+ clauses can share edges.
This means that in matches returned by \autoref{lst:alldifferent} $\atom{k1}$ and $\atom{k2}$ are required to be different, while in matches returned by \autoref{lst:non-unique-edges} $\atom{k1}$ and $\atom{k2}$ are allowed to be equal.

\listingcypher{alldifferent}{Different edges}

\listingcypher{non-unique-edges}{Non-unique edges}

For vertices, this restriction does not apply.\footnote{Requiring uniqueness of edges is often called \emph{edge isomorphic matching}. Other matching strategies, such as \emph{vertex isomorphic matching} (requiring uniqueness of vertices), \emph{isomorphic matching} (requiring uniqueness of both vertices and edges) and \emph{homomorphic matching} (not requiring uniqueness for either) are also used~\cite{DBLP:conf/sigmod/Junghanns17}.} This is illustrated in \autoref{lst:triangle} which returns adjacent persons who like the same message.

\listingcypher{triangle}{Triangle}

\subsubsection{Creating resultset.}

Resultset of a query is basically given in the \lstinline+RETURN+ clause\footnote{Later we will show that for non-last subqueries, one can use \lstinline+WITH+ and also there is az \lstinline+UNWIND+ clause to manipulate resultset.}, which can be de-duplicated using the \lstinline+DISTINCT+ modifier, sorted using the \lstinline+ORDER BY+ subclause. Skipping rows after sorting and limiting the resultset to a certain number of record can be achieved using \lstinline+SKIP+ and \lstinline+LIMIT+ modifiers.

\autoref{lst:duplicate-elimination-sorting} illustrates these concept by returning languages spoken by different persons. The result set is restricted to the third language in alphabetical order.

\listingcypher{duplicate-elimination-sorting}{Deduplicate and sort}

\listingcypher{join}{Multiple patterns}

\subsubsection{Join of patterns.}

Multiple patterns in the same or in different \lstinline+MATCH+ clauses are combined together on variables they share. \autoref{lst:join} illustrates this showing two patterns on lines 2 and 3. First pattern describes a message $\atom{m}$ that has at least two likes.\footnote{Note that the two likes map to different edges according to the uniqueness discussed.} Second pattern finds replies to these messages.

\subsubsection{Aggregation.}
\label{sec:aggregation}

\opencypher specifies aggregation operators for performing calculations on multiple tuples.\footnote{\opencypher has the following grouping functions: \texttt{avg} \texttt{collect} \texttt{count} \texttt{max} \texttt{min} \texttt{percentileCont} \texttt{percentileDisc} \texttt{stdDev} \texttt{stdDevP} \texttt{sum}. All grouping functions return a single scalar value, except \texttt{collect} which returns a list.} Unlike in SQL queries, \emph{grouping criteria} is determined implicitly in the \lstinline+RETURN+ as well as in \lstinline+WITH+ clauses: it contains all vertices, edges and properties that appear outside the grouping functions.

Aggregation is illustrated on \autoref{lst:grouping} which counts the number of persons commanding each language.

\subsubsection{Unwinding a list.}


The \lstinline+UNWIND+ construct takes an attribute and multiplies each tuple replacing the list with the list elements one by one. Because replacing one of the tuple positions, this clause modifies the schema of the subquery. Applying \lstinline+UNWIND+ to the $\atom{speaks}$ attribute (\autoref{lst:unwind}) lists persons along the languages they speak. \autoref{fig:unwind} shows the output of this query. As Cecil speaks two languages, he appears twice in the output. Note that ``Daisy'' speaks no languages, thus no tuples belong to her in the output.

\listingcypher{unwind}{Unwind}

\begin{table}
	\begin{tabular}{|l|c|}
		\hline
		\bf p.name & \bf lang \\ \hline\hline
		Alice & en \\ \hline
		Bob & fr \\ \hline
		Cecil & en \\ \hline
		Cecil & de \\ \hline
	\end{tabular}
	\caption{Output of the query.}
	\label{fig:unwind}
\end{table}

\subsection{Query Structure}

In \opencypher a query is composed as the \lstinline+UNION+ of one or more query parts. Each query part must have the same resulting schema, i.e. the resulting tuples must have the same arity and the same name at each position.

\subsubsection{Query parts.} A single query part is composed of one or more subqueries written subsequently. Subqueries that form a prefix of a regular query have a single result set with the schema of the last subquery's schema in that prefix.

\subsubsection{Subqueries.} Clause sequence of a single subquery matches the regular expression as follows: \mbox{\lstinline+MATCH*((WITH UNWIND?)|UNWIND|RETURN)+}. They begin with an arbitrary number of \lstinline+MATCH+ clauses, followed by either (1)~\lstinline+WITH+ and an optional \lstinline+UNWIND+, (2)~a single \lstinline+UNWIND+, or (3)~a \lstinline+RETURN+ in case of the last subquery.\footnote{In \opencypher, the filtering \lstinline+WHERE+ operation is a subclause of \lstinline+MATCH+ and \lstinline+WITH+. When used in \lstinline+WITH+ as illustrated on line 3 of \autoref{lst:multiple-subqueries}, \lstinline+WHERE+ is similar to the \lstinline+HAVING+ construct of SQL with the major difference that, in \opencypher it is also allowed when no aggregation was specified in the query.}

The \lstinline+RETURN+ and \lstinline+WITH+ clauses use similar syntax and have the same semantics, the only difference being that \lstinline+RETURN+ should be used in the last subquery while \lstinline+WITH+ should only appear in the preceding ones. These clauses list expressions whose value form the tuples, thus they determine the schema of the subquery.

\listingcypher{multiple-subqueries}{Single query part with multiple subqueries}

\begin{table}
	\centering
	\begin{tabular}{|c|c|}
		\hline
		\bf reply & \bf orig \\ \hline\hline
		fr & en \\ \hline
	\end{tabular}
	\caption{Result.}
	\label{fig:multiple-subqueries-result}
\end{table}

\subsubsection{Example.} An \opencypher query of a single query part composed of two subqueries is shown on \autoref{lst:multiple-subqueries} along with its result on \autoref{fig:multiple-subqueries-result}. It retrieves the language of messages that were written in a language no other message uses. If that message was a reply, the language of the original message is also retrieved.

The first subquery spans lines 1--3 and the second spans lines 4--6. The result of the first subquery is a single tuple $\tuple{\atom{``fr"}, 1}$ with the schema $\tuple{\atom{singleLang}, \atom{cnt}}$. The second subquery takes this result as an input to retrieve messages of the given languages and in case of a reply the original message in $\atom{m3}$. 

The result of these two subqueries together produces the final result whose schema is determined by the \lstinline+RETURN+ of the last subquery (line 6).




==> output/alldifferent-gra.tex <==
$
\projection{\var{p1}, \var{k1}, \var{p2}, \var{k2}, \var{p3}
}{}
\alldifferent{\var{k1}, \var{k2}}
\expandout{p2}{p3}{}{k2}{KNOWS}{1}{1}
\expandout{p1}{p2}{}{k1}{KNOWS}{1}{1}
\getvertices{p1}{}
$


==> output/duplicate-elimination-sorting-gra.tex <==
result?

==> output/getvertices-fra.tex <==
$\projection{\atom{p.name}} \selection{\atom{p.age} > 25} \getvertices{p}{Person\,\{name,\,age\}}$


==> output/getvertices-jra.tex <==
$\projection{\atom{p.name}} \selection{\atom{p.age} > 25} \getvertices{p}{Person}$

==> output/join-gra.tex <==
\begin{align*}
\begin{autobreak}
\projection{\var{r}
}{}
%\Big(
\alldifferent{\var{\_e1}, \var{\_e2}, \var{\_e3}}\bigg(
\Big(
\expandin{m}{\_v2}{}{\_e2}{LIKES}{1}{1}
\expandout{\_v1}{m}{Message}{\_e1}{LIKES}{1}{1}%\Big(
\getvertices{\_v1}{}
%\Big)
\Big)
\join
\Big(
\expandin{m}{r}{}{\_e3}{REPLY}{1}{1}%\Big(
\getvertices{m}{Message}
\Big)
\bigg)
%\Big)
\end{autobreak}
\end{align*}


==> output/non-unique-edges-gra.tex <==
$
\projection{\var{p1}, \var{p2}, \var{p3}
}{}
\bigg(
\Big(
\expandboth{p1}{p2}{}{\_e1}{KNOWS}{1}{1}
\getvertices{p1}{}
\Big)
\join
\,
\Big(
\expandboth{p2}{p3}{}{\_e2}{KNOWS}{1}{1}
\getvertices{p2}{}
\Big)
\bigg)
$


==> output/selection1-gra.tex <==
$
\projection{\var{p1.name}, \var{p2.name}
}{}
\selection{
	\var{k.since} < \literal{2000}
}
\expandboth{p1}{p2}{Person}{k}{KNOWS}{1}{1}
\getvertices{p1}{Person}
$

==> output/selection2-gra.tex <==
$
\projection{\var{p.speaks}
}{}
\selection{
	\var{p.name} = \literal{"Bob"}
}
\getvertices{p}{Person}
$

==> output/unwind-gra.tex <==
$
\projection{\var{p.name}, \var{lang}
}{}
\unwind{\var{p.speaks} \assign \var{lang}}
\projection{\var{p}
}{}
\getvertices{p}{Person}
$

==> property-graph-example.tex <==
\footnotesize
\begin{minipage}{0.55\linewidth}
$V = \{a, b, c, d, e, f\}; E=\{1, 2, 3, 4, 5, 6, 7\}$

$\verticestoedges(1) = \tuple{a, b}; \verticestoedges(2) = \tuple{b, c}; \ldots$

$\vertexlabels = \{\atom{Person}, \atom{Message}, \atom{Post}, \atom{Comment}\};$

$\edgelabels = \{\atom{KNOWS}, \atom{LIKES}, \atom{REPLY\_OF}\}$

$\vertexlabelfunction(a) = \{\atom{Person}\}; \vertexlabelfunction(d) = \{\atom{Message}, \atom{Post}\}; \ldots$

$\edgelabelfunction(1) = \atom{KNOWS}; \edgelabelfunction(3) = \atom{LIKES}; \ldots$

$\vertexproperties = \{\atom{name}, \atom{speaks}, \atom{language}\};$

$\edgeproperties = \{\};$

$\propertyfunction{name}{a} = \atom{'Alice'}; \propertyfunction{name}{b} = \atom{'Bob'}; \ldots$

$\propertyfunction{title}{1} = \relnull; \propertyfunction{title}{2} = \atom{}; \ldots$

$\propertyfunction{release}{1} = \relnull; \propertyfunction{release}{2} = \atom{}; \ldots$
\end{minipage}


==> relalg/alldifferent-gra.tex <==
$
\projection{\var{p1}, \var{k1}, \var{p2}, \var{k2}, \var{p3}
}{}
\alldifferent{\var{k1}, \var{k2}}
\expandout{p2}{p3}{}{k2}{KNOWS}{1}{1}
\expandout{p1}{p2}{}{k1}{KNOWS}{1}{1}
\getvertices{p1}{}
$


==> relalg/duplicate-elimination-sorting-gra.tex <==
$
\topp{1}{2}
\sort{\asc \var{p.name}}
\duplicateelimination
\unwind{\vertexlabelfunction(\atom{p}) \assign \atom{label}}
\getvertices{p}{Person}
$

$
\topp{1}{2}
\sort{\asc \var{p.name}}
\duplicateelimination
\unwind{\vertexlabelfunction(\atom{p}) \assign \atom{label}}
\getvertices{p}{Person\,\{\vertexlabelfunction\}}
$


==> relalg/getvertices-fra.tex <==
$
\projection{\var{p}.\atom{name}}
\selection{\var{p}.\atom{age} > 25}
\left(
\getvertices{p}{Person\,\{name,\,age\}}
\right)
$


==> relalg/getvertices-jra.tex <==
$
\projection{\var{p}.\atom{name}}
\selection{\var{p}.\atom{age} > 25}
\left(
\getvertices{p}{Person}
\right)
$

==> relalg/join-gra.tex <==
\begin{align*}
\begin{autobreak}
\projection{\var{r}
}{}
%\Big(
\alldifferent{\var{\_e1}, \var{\_e2}, \var{\_e3}}\bigg(
\Big(
\expandin{m}{\_v2}{}{\_e2}{LIKES}{1}{1}
\expandout{\_v1}{m}{Message}{\_e1}{LIKES}{1}{1}%\Big(
\getvertices{\_v1}{}
%\Big)
\Big)
\join
\Big(
\expandin{m}{r}{}{\_e3}{REPLY}{1}{1}%\Big(
\getvertices{m}{Message}
\Big)
\bigg)
%\Big)
\end{autobreak}
\end{align*}


==> relalg/multihop-fra.tex <==
$
\projection{\var{c}.\atom{name}, \var{scs}, \var{sc}.\atom{name}}
\left(
\left(\getvertices{p1}{Person}\right)
\transitivejoin{1}{\infty}
\left[\getedgesdirected{p1}{Person}{p2}{Person}{sc}{SC\_OF}\right]
\right)
$


==> relalg/multihop-jra.tex <==
$
\projection{\var{c}.\atom{name}, \var{scs}, \var{sc}.\atom{name}}
\left(
\expandout{p1}{p2}{Person}{ks}{SUBCLASS\_OF}{1}{\infty}
\left(\getvertices{p1}{Person}\right)
\right)
$


==> relalg/non-unique-edges-gra.tex <==
$
\projection{\var{p1}, \var{p2}, \var{p3}
}{}
\bigg(
\Big(
\expandboth{p1}{p2}{}{\_e1}{KNOWS}{1}{1}
\getvertices{p1}{}
\Big)
\join
\,
\Big(
\expandboth{p2}{p3}{}{\_e2}{KNOWS}{1}{1}
\getvertices{p2}{}
\Big)
\bigg)
$


==> relalg/selection1-gra.tex <==
$
\projection{\var{p1.name}, \var{p2.name}}
\selection{\var{k.since} < \literal{2000}}
\expandboth{p1}{p2}{Person}{k}{KNOWS}{1}{1}
\getvertices{p1}{Person}
$


==> relalg/selection2-gra.tex <==
$
\projection{\var{p.speaks}}
\selection{	\var{p.name} = \literal{"Bob"}}
\getvertices{p}{Person}
$

==> relalg/unwind-gra.tex <==
$
\projection{\var{p.name}, \var{lang}}
\unwind{\var{p}.\atom{speaks} \assign \var{lang}}
\projection{\var{p}}
\getvertices{p}{Person}
$

==> running-example-formalised.tex <==
\begin{align*}
\vertexlabels &= \{\atom{Person}, \atom{Student}, \atom{Teacher}, \ldots \}\\
\edgelabels &= \{\atom{KNOWS}, \atom{LIKES}, \atom{REPLY\_OF}\}\\
\vertexproperties &= \{\atom{name}, \atom{speaks}, \atom{language}\}\\ \edgeproperties &= \{\atom{since}\}\\
V &= \{a, b, c, d, e, f, g\}\\
E &= \{1, 2, 3, 4, 5, 6, 7\}\\
\verticestoedges&:\ 1 \assign \tuple{a, b}, 2 \assign \tuple{b, c}, \ldots\\
\vertexlabelfunction&:\ b \assign \{\atom{Person}\}, d \assign \{\atom{Message}, \atom{Post}\}, \ldots\\
\edgelabelfunction&:\ 1 \assign \atom{KNOWS}, 3 \assign \atom{LIKES}, \ldots\\
\atom{name}&:\ a \assign \atom{``Alice"}, b \assign \atom{``Bob"}, e \assign \relnull, \ldots\\
\atom{since}&:\ 1 \assign \atom{2011}, 2 \assign \atom{1979}, 3 \assign \relnull, \ldots
\end{align*}



==> table-operators.tex <==
\newcommand{\explanation}[1]{{\small \it (#1)}}

\setlength\tabcolsep{3.6pt}
\begin{table*}[htb]
  \renewcommand\arraystretch{1.15}
  \centering
	\begin{tabular}{@{}lll>{\ttfamily \small}l<{}@{}}
		\toprule
		                              & \multicolumn{1}{c}{\bf Operator}                                                              & \multicolumn{1}{c}{\bf Name} & \multicolumn{1}{c}{\bf openCypher code}     \\ \midrule
		\multirow{9}{*}{GRA}          & $\expandout{\atom{v}}{\atom{w}}{W}{e}{E}{1}{1} (r)$                                           & \expandouttext               & (v) -[e:E]->(w:W)                           \\
		                              & $\expandin{\atom{v}}{\atom{w}}{W}{e}{E}{1}{1} (r)$                                            & \expandintext                & (v)<-[e:E]- (w:W)                           \\
		                              & $\expandboth{\atom{v}}{\atom{w}}{W}{e}{E}{1}{1} (r)$                                          & \expandbothtext              & (v) -[e:E]- (w:W)                           \\
		                              & $\expandout{\atom{v}}{\atom{w}}{W}{e}{E*}{1}{1} (r)$                                          & \expandouttext transitive    & (v) -[e:E*]->(w:W)                          \\
		                              & $\expandin{\atom{v}}{\atom{w}}{W}{e}{E*}{1}{1} (r)$                                           & \expandintext transitive     & (v)<-[e:E*]- (w:W)                          \\
		                              & $\expandboth{\atom{v}}{\atom{w}}{W}{e}{E*}{1}{1} (r)$                                         & \expandbothtext transitive   & (v) -[e:E*]- (w:W)                          \\
		\multirow{17}{*}{GRA/JRA/FRA} & $\getvertices{v}{V}$                                                                          & \getverticestext             & (v:V)                                       \\
		                              & $\getedgesdirected{v}{}{w}{}{e}{}$                                                            & \getedgestext                & (v:V)-[e:E]->(w:W)                          \\
		                              & $\alldifferent{\atom{vars}} (r)$                                                              & \alldifferenttext            & \explanation{default matching semantics}    \\
		                              & $\unwind{\atom{xs} \assign \atom{x}} (r)$                                                     & \unwindtext                  & \lstinline+UNWIND+                          \\
		                              & $\selection{\atom{condition}} (r)$                                                            & \selectiontext               & \lstinline+WHERE+                           \\
		                              & $\projection{\atom{x_1}, \atom{x_2}, \ldots}{} (r)$                                           & \projectiontext              & \lstinline+WITH, RETURN+                    \\
		                              & $\grouping{\atom{x_1}, \atom{x_2}, \ldots}{\atom{c_1}, \atom{c_2}, \ldots} (r)$               & \groupingtext                & \lstinline+WITH, RETURN+                    \\
		                              & $\production{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                             & \productiontext              & \lstinline+RETURN+                          \\
		                              & $\duplicateeliminationop (r)$                                                                 & \duplicateeliminationtext    & \lstinline+DISTINCT+                        \\
		                              & $\sort{\desc \atom{x_1}, \asc \atom{x_2}, \ldots} (r)$                                        & \sorttext                    & \lstinline+ORDER BY+                        \\
		                              & $\topp{\atom{skip}}{\atom{limit}} (r)$                                                        & \toptext                     & \lstinline+SKIP, LIMIT+                     \\
		                              & $r \unionop s$                                                                                & \uniontext                   & \lstinline+UNION+                           \\
		                              & $r \bagunion s$                                                                               & \baguniontext                & \lstinline+UNION ALL+                       \\
		                              & $r \joinop s$                                                                                 & \jointext                    & \lstinline+WITH+                            \\
		                              & $r \leftouterjoin s$                                                                          & \leftouterjointext           & \lstinline+OPTIONAL MATCH+                  \\
		                              & $r \thetaleftouterjoin s$                                                                     & \thetaleftouterjointext      & \lstinline+OPTIONAL MATCH ... WHERE+        \\
		                              & $r \antijoinop s$                                                                             & \antijointext                & \lstinline+WHERE NOT+ \explanation{pattern} \\ \midrule
		\multirow{2}{*}{JRA/FRA}      & $\sortop \topop_{\desc \atom{x_1}, \asc \atom{x_2}, \ldots}\ _\atom{skip}^{\atom{limit}} (r)$ & \sortandtoptext              & \lstinline+ORDER BY ... SKIP ... LIMIT+     \\
		                              & $r \transitivejoinop_{[e]} s$                                                                 & \transitivejointext          & \\ \midrule
		\multirow{5}{*}{modification} & $\delete{\atom{[detach]}}{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                & \deletetext                  & \lstinline+[DETACH] DELETE+                 \\
		                              & $\create{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                                 & \createtext                  & \lstinline+CREATE+                          \\
		                              & $\mergenode{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                              & \mergetext                   & \lstinline+MERGE+                           \\
		                              & $\removenode{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                             & \removetext                  & \lstinline+REMOVE+                          \\
		                              & $\setnode{\atom{x_1}, \atom{x_2}, \ldots} (r)$                                                & \settext                     & \lstinline+SET+                             \\
		%
    \bottomrule             &
	\end{tabular}
	\caption{Operators of the extended relation algebras.}
\label{table:operators}
\end{table*}

